Electrical networks and hyperplane arrangements

This paper studies \emph{Dirichlet arrangements}, a generalization of graphic hyperplane arrangements arising from electrical networks and order polytopes of finite posets. We generalize descriptions of combinatorial features of graphic arrangements to Dirichlet arrangements, including characteristic polynomials and supersolvability. We apply these results to visibility sets of order polytopes and fixed-energy harmonic functions on electrical networks.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

This paper studies a class of hyperplane arrangements with connections to electrical networks and order polytopes of finite posets. Consider a graph $\g=(V,E)$ equipped with an independent set $\B\subset V$ of $\geq 2$ \emph{nodes} and an injective function $\u:\B\to \R$. The pair $(\g,\u)$ represents an electrical network if one considers the edges $E$ as linear resistors of equal conductance and the values of $\u$ as fixed voltages on the nodes. By assigning edge weights $\con\in \C^E$ one can represent networks of more general electrical components, such as RLC circuits.

For generic $\con$ the triple $(\g,\u,\con)$ determines a unique harmonic function $h:V\to \R$ extending $\u$. In this scenario the \emph{energy} dissipated by a resistor $ij\in E$ is given by
\begin{equation}
	\eng_{ij}=\con_{ij}(h(i)-h(j))^2.
\end{equation}	
Given a network $(\g,\u)$ and fixed energies $\eng\in \C^E$, one can ask which $\con\in \C^E$ produce the energies $\eng$. Equivalently, one can consider the harmonic functions $h$ associated to these $\con$, called \emph{$\eng$-harmonic functions} on $(\g,\u)$.

\begin{prob}
	Given a network $(\g,\u)$ and fixed energies $\eng\in \C^E$, describe the set of $\eng$-harmonic functions on $(\g,\u)$.
	\label{prob:eharm}
\end{prob}

Abrams and Kenyon \cite{abrams2016} showed that if $\eng\in (0,\infty)^E$, then the $\eng$-harmonic functions on $(\g,\u)$ are real-valued, and that the number of $\eng$-harmonic functions is the same for generic $\eng\in \C^E$. We generalize these observations as follows.

\begin{thm}
	The $\eng$-harmonic functions on $(\g,\u)$ are the critical points of a master function of a real hyperplane arrangement $\Au$.
	\label{thm:cpchar}
\end{thm}

Broadly speaking, critical points of master functions generalize analytic centers of convex polytopes. Master functions and their critical points form an active area of research with applications to Lie algebras, physics, integrable systems, and algebraic geometry \cite{cohen2011, huh2013, mukhin2005, varchenko2011, varchenko2014}. Thus Theorem \ref{thm:cpchar} connects Problem \ref{prob:eharm} to an existing body of results from the theory of hyperplane arrangements. For example, a foundational theorem of Varchenko \cite{varchenko1995} implies that if $\eng\in (0,\infty)^E$, then there is one $\eng$-harmonic function in each bounded chamber of $\Au$, and there are no others.

In Section \ref{sec:master} we define the arrangement $\Au$, called a \emph{Kirchhoff arrangement}. We then prove Theorem \ref{thm:cpchar}, obtaining the results of Abrams and Kenyon \cite{abrams2016} as corollaries. Many desirable features of graphic arrangements can be extended to Kirchhoff arrangements in interesting ways, despite core structural differences between the two classes. Here we present some of the most fundamental examples, deferring more specialized results to future articles \cite{lutz2018kos,lutz2018mat}.

\begin{thm}
	Consider the Kirchhoff arrangement $\Au$, and let $\mg$ be the graph obtained from  $\g$ by adding an edge between each pair of nodes. The following hold:
	\begin{enumerate}[(i)]
		\item The intersection poset of $\Au$ is isomorphic to the poset of node-separating connected partitions of $\g$
		\item The characteristic polynomial of $\Au$ is the quotient of the chromatic polynomial of $\mg$ by a falling factorial
		\item The bounded chambers of $\Au$ correspond to the orientations of possible current flows through the network $(\g,\u)$
		\item The arrangement $\Au$ is supersolvable if and only if $\mg$ is chordal.
	\end{enumerate}
	\label{thm:maincomb}
\end{thm}

In Section \ref{sec:combo} we prove Theorem \ref{thm:maincomb} and several related results of interest. For example, we show that the coefficients of a chromatic polynomial remain log-concave after ``modding out'' by any clique of the graph. We also obtain a formula for the number of bounded chambers of $\Au$ in terms of the beta invariant of $\mg$.

Apart from their connection to electrical networks, one reason to study Kirchhoff arrangements is that they are equivalent to \emph{$\psi$-graphical arrangements}, introduced by Stanley \cite{stanley2015} to study order polytopes of finite posets. Our definition provides a more natural viewpoint on these arrangements, leading to simpler descriptions of their combinatorics. For example, the literature on $\psi$-graphical arrangements so far has centered on characterizing their supersolvability \cite{mu2015,stanley2015,suyama2018}; Theorem \ref{thm:maincomb}(iv) gives a pleasing graph-theoretic characterization that closely resembles the analogous result for graphic arrangements. We prove the equivalence of the two classes in Section \ref{sec:super}.

In the appendix we elaborate on an observation of Abrams and Kenyon that if $\eng\in (0,\infty)^E$, then $\Gal(\Qtr/\Q)$ acts on the set of $\eng$-harmonic functions on $(\g,\u)$, where $\Qtr$ is the field of totally real numbers. We exhibit an action of $\Gal(\Qtr/\Q)$ on the critical points of any master function of a real arrangement with positive weights.

==> sections/intro2-els.tex <==
\section{Introduction}
\label{sec:intro}

The \emph{graphic arrangement} associated to a graph $\g=(V,E)$ is the set $\Ag$ of hyperplanes in $\R^V$ given by $x_i=x_j$ for all $ij\in E$. Graphic arrangements are fundamental in the study of hyperplane arrangements due to the relative ease of translating combinatorial and topological data from $\Ag$, often intractable for general arrangements, into graph-theoretic terms.

This paper studies \emph{Dirichlet arrangements}, a generalization of graphic arrangements arising from electrical networks and order polytopes of finite posets.
%We show that the main combinatorial features of Dirichlet arrangements generalize those of graphic arrangements in interesting and user-friendly ways. As applications, we characterize harmonic functions on electrical networks as critical points of master functions in the sense of Varchenko, and we give a simple formula for the number of visibility sets of an order polytope.
Let $\g$ be a finite connected undirected graph with no loops or multiple edges. Let $\B\subset V$ be a set of $\geq 2$ vertices called \emph{boundary nodes}, no two of which are adjacent. Let $ u:\B\to \R$ be injective. We think of $\g$ as a network of linear resistors with voltages $ u$ imposed on the boundary nodes. The \emph{Dirichlet arrangement} $\Au$ is the set of intersections of hyperplanes in the graphic arrangement $\Ag$ with the affine subspace
\begin{equation}
\{x\in \R^V:x_j =  u(j)\mbox{ for all }j\in \B\}.
\label{eq:affsub}
\end{equation}
The Dirichlet arrangement $\Au$ is not a genuine restriction of $\Ag$, since \eqref{eq:affsub} is not an intersection of elements of $\Ag$. %In general there is little combinatorial resemblance between an arrangement $\AA$ and an arbitrary affine slice of $\AA$.
However we show that $\Au$ preserves a good deal of graphic structure.

\begin{thm}
	Let $\mg$ be the graph obtained from $\g$ by adding an edge between each pair of boundary nodes. The following hold:
	\begin{enumerate}[(i)]
		\item The intersection poset $L(\Au)$ is the order ideal of $L(\Ag)$ consisting of all boundary-separating connected partitions of $\g$
		\item The characteristic polynomial of $\Au$ is the quotient of the chromatic polynomial of $\mg$ by a falling factorial
		\item The bounded chambers of $\Au$ correspond to the possible orientations of current flow through $\g$ respecting the voltages $u$ and in which the current flowing through each edge is nonzero.
	\end{enumerate}
	\label{thm:maincomb}
\end{thm}

Each part of Theorem \ref{thm:maincomb} generalizes a key theorem on graphic arrangements. As corollaries, we obtain a formula for the number of orientations in part (iii), and we show that the coefficients of a chromatic polynomial remain log-concave after ``modding out'' by a clique of the graph.

We also characterize supersolvable Dirichlet arrangements. %Supersolvable arrangements are desirable in part because their characteristic polynomials and related algebras factor nicely.
Stanley \cite{stanley1972} showed that the graphic arrangement $\Ag$ is supersolvable if and only if the graph $\g$ is chordal (or triangulated). We prove the following theorem, building on results of \cite{mu2015,stanley2015,suyama2018}.

\begin{thm}
	The Dirichlet arrangement $\Au$ is supersolvable if and only if the graph $\mg$ from Theorem \ref{thm:maincomb} is chordal.
	\label{thm:supintro}
\end{thm}

This answers a question posed by Stanley \cite{stanleytalk}, who asked if there is a characterization of supersolvable arrangements $\Au$ analogous to the graphic case (see Section \ref{sec:super}).

For an application of our results, let $P$ be a finite poset and $O$ the convex polytope in $\R^P$ of all order-preserving functions $P\to [0,1]$. Here $O$ is called the \emph{order polytope} of $P$ \cite{stanley1986}. %The \emph{visibility arrangement} of $O$ is the set $\AA(O)$ of affine spans of facets of $O$. The chambers of $\AA(O)$ correspond to
Consider the sets of facets of $O$ visible from different points in $\R^P$, called \emph{visibility sets} of $O$. In general not all visibility sets of $O$ are visible from far away, since certain obstructions are eliminated by viewing $O$ ``from infinity.'' Write $\alpha(\g)$ and $\beta(\g)$ for the number of acyclic orientations and the beta invariant, resp., of $\g$.

\begin{cor}
	Let $O$ be the order polytope of a finite poset. There is a graph $\Delta$ such that $O$ has exactly $\frac{1}{2}\alpha(\Delta)$ visibility sets, of which exactly $\frac{1}{2}\alpha(\Delta)-\beta(\Delta)$ are visible from far away.
	\label{cor:vis}
\end{cor}

Another application involves electrical networks with fixed boundary voltages. The pair $(\g, u)$ represents such a network if we consider the edges $E$ as resistors of equal conductance. By assigning complex edge weights $\con\in \C^E$ we can represent networks involving more general electrical components, such as RLC circuits.

For generic $\con\in \C^E$ the triple $(\g, u,\con)$ determines a unique harmonic function $h:V\to \C$ extending $ u$. In this scenario the \emph{energy} dissipated by a resistor $ij\in E$ is given by
\begin{equation}
\eng_{ij}=\con_{ij}(h(i)-h(j))^2.
\end{equation}	
Given a network $(\g, u)$ and fixed energies $\eng\in \C^E$, it is natural to ask which conductances $\con\in \C^E$ produce the energies $\eng$. Abrams and Kenyon \cite{abrams2016} posed the equivalent problem of describing the set of harmonic functions associated to these $\con$, called \emph{$\eng$-harmonic functions} on $(\g, u)$.

We describe the $\eng$-harmonic functions on $(\g,u)$ as critical points of \emph{master functions} of $\Au$ in the sense of Varchenko \cite{varchenko2003}. Broadly, master functions generalize logarithmic barrier functions, and their critical points generalize analytic centers of systems of linear inequalities.

\begin{thm}
	The $\eng$-harmonic functions on $(\g, u)$ are the critical points of the master function of $\Au$ with weights $\eng$.
	\label{thm:cpchar}
\end{thm}

Theorem \ref{thm:cpchar} connects electrical networks, a subject with a vast literature \cite{brooks1940, curtis2000, postnikov2006, seshu1961, smale1972, weyl1923}, to critical points of master functions, an active area of research with applications to Lie algebras, physics, integrable systems, and algebraic geometry \cite{cohen2011, huh2013, mukhin2005, varchenko2011, varchenko2014}. We obtain results of Abrams and Kenyon \cite{abrams2016} as corollaries of Theorem \ref{thm:cpchar}. Combining these results with Theorem \ref{thm:maincomb} yields the following.

\begin{cor}
	For generic $\eng$, the number of $\eng$-harmonic functions is
	\[\frac{\beta(\mg)}{(|\B|-2)!}.\]
	\label{cor:eharmcount}
\end{cor}

The paper is organized as follows. In Section \ref{sec:maindef} we establish basic properties and examples of Dirichlet arrangements. In Section \ref{sec:combo} we prove Theorem \ref{thm:maincomb}. In Section \ref{sec:super} we prove Theorem \ref{thm:supintro} and discuss the relationship of Dirichlet arrangements to previous work \cite{mu2015, stanley2015, suyama2018}. In Section \ref{sec:master} we prove Theorem \ref{thm:cpchar}. In the appendix we exhibit an action of $\Gal(\Qtr/\Q)$ on the critical points of any master function with positive rational weights, where $\Qtr$ is the field of totally real numbers.

==> sections/maindef-els.tex <==
\section{Dirichlet arrangements}
\label{sec:maindef}
	
	Given a base field $\KK$, an \emph{arrangement} $\AA$ in $\KK^d$ is a finite set of affine hyperplanes of $\KK^d$. We consider each arrangement $\AA$ in $\KK^d$ to be equipped with a set $\{f_H : H\in\AA\}$ of affine functionals $f_H:\KK^d\to\KK$ such that $H=\ker f_H$ for all $H\in \AA$. The $f_H$ are called \emph{defining functions} of $\AA$. We write
	\[Q(\AA)=\prod_{H\in \AA} f_H(x).\]
	
	An arrangement $\AA$ is \emph{defined over} a subring $S\subset \KK$ if in the standard basis of $\KK^d$ all coefficients of all defining functions $f_H$ belong to $S$. We write 
	\[T(\AA)=\bigcap_{H\in \AA} H\]
	if $\AA$ is nonempty and $T(\emptyset)=\KK^d$. We also write $M(\AA)=\KK^d\setminus \bigcup_{H\in \AA} H$. When $\KK=\R$, the connected components of $M(\AA)$ are called the \emph{chambers} of $\AA$. The arrangement $\AA$ is called \emph{central} if $T(\AA)$ is nonempty and \emph{essential} if the normal vectors of $\AA$ span $\KK^d$. The \emph{cone} $c\AA$ over $\AA$ is the central arrangement in $\KK^{d+1}$ defined by
	\[Q( c\AA) = x_0\prod_{H\in \AA} {f^h_H(x_0,\ldots,x_d)},\]
	where $f^h_H$ is the homogenization of $f_H$ with respect to the new variable $x_0$.

	\subsection{Dirichlet arrangements}
	
	By a \emph{graph} we will mean one that is finite, connected and undirected with no loops or multiple edges. Denote by $\g=(V,E)$ a graph on $d$ vertices and $k$ edges. The \emph{graphic arrangement} $\Ag$ of $\g$ over a field $\KK$ is the arrangement in $\KK^d$ defined by
	\[Q(\Ag)=\prod_{ij\in E} (x_i-x_j).\]
	
	Fix a set $\B\subsetneq V$ of $\geq 2$ vertices, no two of which are adjacent, and an injective function $u:\B\to \KK$. We call $\B$ the \emph{boundary} of $\g$ and $\inte=V\setminus \B$ the \emph{interior} of $\g$. We call $ u$ the \emph{boundary data} and the scalars $ u(j)\in\KK$ the \emph{boundary values}. The elements of $\B$ are called \emph{boundary nodes}. Write $m=|\B|$ and $n=|\inte|$, so $d=m+n$. Whenever the vector spaces $\KK^d$ and $\KK^n$ appear, we consider their coordinates to be indexed by $V$ and $\inte$, resp.
	
	\begin{mydef}
		Let $\Au$ be the arrangement in
		\[\XX=\{x\in \KK^d : x_j =  u(j)\mbox{ for all }j\in \B\}\cong \KK^n\]
		of hyperplanes $H\cap \XX$ for all $H\in \Ag$. An arrangement $\AA$ is \emph{Dirichlet} if $\AA=\Au$ for some $(\g, u)$.
		\label{def:Au}
	\end{mydef}

	This definition can be relaxed to include $m=0$, in which case $\Au=\Ag$ is graphic, and $m=1$, in which case $\Au$ has the same underlying combinatorics as $\Ag$. We restrict our attention to $m\geq 2$ in order to distinguish our results from the graphic cases. For example, graphic arrangements are central but not essential, but we have the following for Dirichlet arrangements.
	
	\begin{prop}
		Dirichlet arrangements are essential but not central.
		
		\begin{proof}
			For each $e\in E$ let $H_e$ be the corresponding element of $\Au$ with normal vector $v_e$ of the form $x_i-x_j$ or $x_i- u(j)x_j$. Since $\g$ is connected, for any $i\in \inte$ there is a path $P\subset E$ with one endpoint $i$ and the other endpoint in $\B$. We have $\sum_{e\in P} v_e = x_i$, replacing some $v_e$ with $-v_e$ if necessary. It follows that the normal vectors span $\KK^n$, so $\Au$ is essential. Since $\g$ is connected, there is a path $Q\subset E$ of between distinct boundary nodes $j$ and $j'$. If $x\in \bigcap_{e\in Q} H_e$, then $ u(j)=x_j=x_{j'}=  u(j')$, a contradiction. Hence $\Au$ is not central.
		\end{proof}
		
		\label{prop:centess}
	\end{prop}
	
	Definition \ref{def:Au} can also be modified to accommodate repeated boundary values and edges between boundary nodes. In case of repeated boundary values, one can identify all vertices on which $ u$ takes the same value, removing any duplicate edges. In case $\B$ is not an independent set, one can simply remove all edges between boundary nodes, assuming that the resulting graph is connected. Then define $\Au$ as in Definition \ref{def:Au}.  
	
	For the remainder of the paper we will assume that $\KK=\R$. We think of $\Au$ as an $n$-dimensional affine slice of $\Ag$, where for all $i\in \inte$ the coordinates $x_i$ of $\XX\cong\R^n$ are inherited from $\R^d$, and for all $j\in \B$ the coordinate $x_j$ is specialized to the boundary value $ u(j)$. 
	
	\begin{eg}[Wheatstone bridge]
		Consider the graph $\g$ on the left side of Figure \ref{fig:dir}, where the boundary nodes $j_1$ and $j_2$ are marked by white circles. The pair $(\g,\B)$ is sometimes called a \emph{Wheatstone bridge} after the work of C.~Wheatstone \cite{wheatstone1843}. A Wheatstone bridge can also be represented by a circuit diagram, as in Figure \ref{fig:dir}; here, jagged edges denote resistors, and the symbol on top denotes a battery between the boundary nodes.
		
		Fix boundary values $ u(j_1)=1$ and $ u(j_2)=-1$. This corresponds to placing a 2-volt battery between the boundary nodes. Writing  $\inte= \{i_1,i_2\}$, the Dirichlet arrangement $\Au$ is defined by
		\[Q(\Au)=(x_{i_1}^2-1)(x_{i_2}^2-1)(x_{i_1}-x_{i_2}).\]
		The bounded chambers of $\Au$ are the open triangles shaded on the right-hand side of Figure \ref{fig:dir}.  
		
		\begin{figure}[ht]
			\centering
			\input{tikz/dir-els}
			\caption{Left to right: a Wheatstone bridge $(\g,\B)$; the associated circuit diagram; and a corresponding Dirichlet arrangement $\Au$.}
			\label{fig:dir}
		\end{figure}
		
		\label{eg:dir}
	\end{eg}

\begin{eg}[Slices of braid arrangements]
	Suppose that $\inte$ is a clique, and that every vertex in $\B$ is adjacent to every vertex in $\inte$. We denote this graph with specified boundary by 
	\[\comp{m}{n}=(\g,\B).\]
	For instance, the Wheatstone bridge in Example \ref{eg:dir} is $\comp{2}{2}$. The case $\comp{5}{4}$ is illustrated in Figure \ref{fig:compjoin} with boundary nodes marked by white circles. Every Dirichlet arrangement is a subset of some $\Au$, where $(\g,\B)=\comp{m}{n}$.
	
	\begin{figure}[ht]
		\centering
		\input{tikz/compjoin}
		\caption{The network $\comp{5}{4}$ with boundary nodes marked in white.}
		\label{fig:compjoin}
	\end{figure}
	\label{eg:compjoin}
\end{eg}

\begin{eg}[Visibility arrangements of order polytopes]
	Let $P$ be a finite poset. The \emph{order polytope} $\mathcal{O}(P)$ of $P$ is the set of all order-preserving functions $P\to [0,1]$. Clearly $\mathcal{O}(P)$ is a convex polytope in $\R^P$. The \emph{visibility arrangement} $\operatorname{vis}(\mathcal{O}(P))$ of $\mathcal{O}(P)$ is the arrangement in $\R^P$ whose elements are the affine spans of all facets of $\mathcal{O}(P)$. It is so named because the chambers of $\operatorname{vis}(\mathcal{O}(P))$ correspond to the sets of facets of $\mathcal{O}(P)$ visible from different points in $\R^P$. Notice that the unbounded chambers of $\operatorname{vis}(\mathcal{O}(P))$ correspond to the sets of facets visible from far away.
	
	Consider the Hasse diagram $H$ of $P$ as a graph, so that the elements of $P$ are the vertices of $H$. Let $\g$ be the graph obtained by adding 2 vertices $j_0$ and $j_1$ to $H$, with $j_0 \sim i$ if $i$ is minimal in $P$ and $j_1\sim i$ if $i$ is maximal in $P$. Let $\B=\{j_0,j_1\}$, and let $ u:\B\to \R$ be given by $ u(j_0)=0$ and $ u(j_1)=1$. Then $\Au=\operatorname{vis}(\mathcal{O}(P))$ (see \cite[Theorem 4]{stanley2015}).
	\label{eg:vis}
\end{eg}

\begin{eg}[Linear order polytope]
	Let $P=\{1,\ldots,\ell\}$ with the usual linear ordering. The weakly increasing maps $P\to [0,1]$ correspond to points $x\in\R^\ell$ with $0\leq x_1 \leq \cdots \leq c_\ell \leq 1$. Thus the order polytope $\mathcal{O}(P)$ is an $\ell$-simplex in $\R^\ell$. Every nonempty subset of the $\ell+1$ facets of $\mathcal{O}(P)$ is a visibility set; by Corollary \ref{cor:vis} we must have $\frac{1}{2}\alpha(\mg)=2^{\ell+1}-1$, where $\mg$ (as defined in Example \ref{eg:vis}) is a cycle graph on $\ell+2$ vertices. The set of all facets is only visible from the interior of $\mathcal{O}(P)$, and is the only set not visible from far away.
\end{eg}

==> tikz/dir2.tex <==
\begin{tikzpicture}
\draw[fill=black!20] (-1,-1) -- (1,-1) -- (1,1) -- (-1,1) -- cycle;
\draw (-1,-1.618) -- (-1,1.618);
\draw (1,-1.618) -- (1,1.618);
\draw (-1.618,-1) -- (1.618,-1);
\draw (-1.618,1) -- (1.618,1);
\draw (-1.618,-1.618) -- (1.618,1.618);
\end{tikzpicture}
